On the Sobolev removability of the graph of one-dimensional Brownian motion

Suppose that $B$ is a one-dimensional Brownian motion and let $\Gamma = \{ (t, B_t) : t \in [0,1]\}$ be the graph of $B|_{[0,1]}$. We characterize the Sobolev removability properties of $\Gamma$ by showing that $\Gamma$ is almost surely not $W^{1,p}$--removable for all $p \in [1, \infty)$ but is almost surely $W^{1,\infty}$--removable.

==> commandsConformalRemovability.tex <==
% Theorem environments
\newtheorem{theorem}{Theorem}[section]

\theoremstyle{definition} % This controls font in theorems & definitions
\newtheorem{definition}[theorem]{Definition}
\newtheorem*{definition*}{Definition}

\theoremstyle{plain}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{cor}[theorem]{Corollary}
\newtheorem{claim}[theorem]{Claim}


\newtheorem*{lemma*}{Lemma}
\newtheorem*{cor*}{Corollary}
\newtheorem*{theorem*}{Theorem}
\newtheorem*{claim*}{Claim}


\renewcommand\qedsymbol{$\square$}


% Auxiliary commands
\DeclareMathSymbol{:}{\mathpunct}{operators}{"3A}%semicolon spaces
\RequirePackage{xspace}
\def\mat#1{\ensuremath{#1}\xspace}
\def\dmat#1#2{\gdef#1{\mat{#2}}}
\def\csdmat#1#2{\csdef{#1}{\mat{#2}}}

\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\res}{res}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\cl}{cl}
\DeclareMathOperator{\Prime}{Prime}
\DeclareMathOperator{\Spec}{Spec}
\DeclareMathOperator{\ord}{ord}
\DeclareMathOperator{\codim}{codim}
\DeclareMathOperator{\range}{range}
\DeclareMathOperator\coker{coker}


\DeclareMathOperator{\sech}{sech}
\DeclareMathOperator{\csch}{csch}
\DeclareMathOperator{\arcsec}{arcsec}
\DeclareMathOperator{\arccot}{arcCot}
\DeclareMathOperator{\arccsc}{arcCsc}
\DeclareMathOperator{\arccosh}{arccosh}
\DeclareMathOperator{\arcsinh}{arcsinh}
\DeclareMathOperator{\arctanh}{arctanh}
\DeclareMathOperator{\arcsech}{arcsech}
\DeclareMathOperator{\arccsch}{arcCsch}
\DeclareMathOperator{\arccoth}{arcCoth} 
\DeclareMathOperator{\tr}{tr} 
\DeclareMathOperator{\Span}{Span}

\newcommand{\N}{\mathbf{N}}
\newcommand{\Z}{\mathbf{Z}}
\newcommand{\Q}{\mathbf{Q}}
\newcommand{\R}{\mathbf{R}}
\newcommand{\C}{\mathbf{C}}
\newcommand{\Ha}{\mathbf{H}}
\renewcommand{\H}{\mathbf{H}}
\newcommand{\D}{\mathbf{D}}
\newcommand{\fk}{\mathbf{k}}
\newcommand{\F}{\mathbf{F}}
\newcommand{\E}{\mathbf{E}}
\renewcommand{\P}{\mathbf{P}}
\newcommand{\M}{\mathbf{M}}


% Mathcal Letters. Usage: \cA
\RequirePackage{etoolbox}
\def\defcal#1{\csdmat{c#1}{\mathcal{#1}}}
\forcsvlist\defcal{A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}

\newcommand{\mb}{\mathbf}

\newcommand{\gl}{GL(n,\R)}
\newcommand{\GL}[1]{GL\left(#1\right)}
\DeclareMathOperator{\SL}{SL}
\newcommand{\sln}{SL(n,\R)}

\newcommand{\qi}{\textbf{i}}
\newcommand{\qj}{\textbf{j}}
\newcommand{\qk}{\textbf{k}}

%Greek
\newcommand{\ee}{\varepsilon}
\newcommand{\dd}{\delta}
\newcommand{\aal}{\alpha}
\newcommand{\bb}{\beta}
\renewcommand{\gg}{\gamma}
\newcommand{\GG}{\Gamma}
\newcommand{\la}{\lambda}
\newcommand{\ff}{\varphi}
\newcommand{\om}{\omega}
\newcommand{\tht}{\theta}
\newcommand{\DD}{\Delta}
\newcommand{\Om}{\Omega}
\newcommand{\kk}{\kappa}
\renewcommand{\ss}{\sigma}

\newcommand{\La}{\Lambda}


\newcommand{\nv}{^{-1}}

\newcommand{\lnti}{\lim_{n\to\infty}}
\newcommand{\lxtz}{\lim_{x\to0}}
\newcommand{\lxtzp}{\lim_{x\to0^+}}
\newcommand{\lxtzm}{\lim_{x\to0^-}}
\newcommand{\tra}{\pitchfork}
\newcommand{\del}{\partial}

\newcommand*{\pdv}[3][]{\frac{\partial^{#1} #2}{\partial #3}}
\newcommand*{\dv}[3][]{\frac{d^{#1} #2}{d#3}}

\newcommand{\lcm}{\text{lcm}}



\newcommand{\bal}{\begin{align*}}
\newcommand{\ealin}{\end{align*}}

\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\rr}{\begin{flushright}}
\newcommand{\er}{\end{flushright}}

\newcommand{\ben}{\begin{enumerate}[label=(\alph*)]}
\newcommand{\een}{\end{enumerate}}
\newcommand{\bren}{\begin{enumerate}[label=\alph*), leftmargin=*]}
\newcommand{\eren}{\end{enumerate}}



\def\n#1{\left\lvert#1\right\rvert}
\def\nn#1{\left\lVert#1\right\rVert}

\def\seq#1{\left\{#1_n\right\}_{n=1}^\infty}
\def\sq#1{\left\{#1_n\right\}}
\def\set#1{\left\{#1\right\}}
\def\muse#1{\mu\left(\left\{#1\right\}\right)}

\newcommand{\defeq}{\stackrel{\text{def}}{=}}

\newcommand{\ev}{\text{ev}}
\newcommand{\interior}[1]{%
{\kern0pt#1}^{\mathrm{o}}%
}

%191 Nonlinear Algebra 
\renewcommand{\vec}{\boldsymbol}
\newcommand{\x}{\vec x}
% \newcommand{\kk}{K[\vec x]}
\newcommand{\gen}[1]{\left\langle #1 \right\rangle}
\newcommand{\init}{\text{in}_{\prec}(I)}
\newcommand{\ini}[1]{\text{in}_{\prec}(#1)}
\DeclareMathOperator{\Jac}{Jac}
\DeclareMathOperator{\rank}{rank}
\newcommand{\rrad}{\sqrt[\R]}
\newcommand{\rri}{\sqrt[\R]{I}}
\newcommand{\rx}{\R[\vec x]}
\newcommand{\cx}{\C[\vec x]}
\DeclareMathOperator{\val}{val}
\DeclareMathOperator{\tdet}{tropdet}
\DeclareMathOperator{\sym}{Sym}

%202b 
\newcommand{\clxsm}{\cL^1(X, \cS, \mu)}
\newcommand{\lxsm}{\L^1(X, \cS, \mu)}
\newcommand{\lox}{\L^1(X)}
\newcommand{\lo}{\L^1}
\DeclareMathOperator{\Lip}{Lip} 
\newcommand{\Cin}{C_\infty(X)}
\newcommand{\inn}[1]{\nn{#1}_\infty}
\newcommand{\clo}[1]{\overline{#1}}
\newcommand{\ccx}{C_c(X)}
\DeclareMathOperator{\supp}{support}

%250b
\DeclareMathOperator{\Ass}{Ass}
\DeclareMathOperator{\Ann}{Ann}
\newcommand{\mx}{\mathfrak m}

%4th Year Project ---------------------------------
\newcommand{\md}{\mathbf{M}^d}

%Interpolation Spaces
\newcommand{\nnc}[1]{\nn{#1}_{X_0 \cap X_1}}
\newcommand{\nnp}[1]{\nn{#1}_{X_0 + X_1}}
\newcommand{\nnz}[1]{\nn{#1}_{X_0}}
\newcommand{\nno}[1]{\nn{#1}_{X_1}}
\newcommand{\nni}[3]{\nn{#3}_{#1,#2}}
\newcommand{\ntq}[1]{\nn{#1}_{\theta, q}}
\newcommand{\xtq}{\left(X_0, X_1\right)_{\theta, q}}
\newcommand{\inc}{\xhookrightarrow{}}

%Sobolev Spaces
\newcommand{\nmp}[1]{\nn{#1}_{m,p}}
\newcommand{\cciu}{C_c^\infty(U)}
\newcommand{\du}{\cD(U)}
\newcommand{\lab}{L^2_{(\aal, \beta)}}
\newcommand{\labn}{L^2_{(\aal + n, \beta + n)}}
\newcommand{\wnab}{W^n_{(\aal, \beta)}}
\newcommand{\wrab}{W^R_{(\aal, \beta)}}
\newcommand{\nnab}[1]{\nn{#1}_{L^2_{(\aal, \beta)}}}
\newcommand{\genab}[1]{\left\langle #1 \right\rangle_{\aal, \beta}}
\newcommand{\ltg}{L^2_{\gg}}
\renewcommand{\wp}{W^{1,p}}
\newcommand{\woi}{W^{1,\infty}}
\newcommand{\wpom}{W^{1,p}(\Omega)}


\newcommand{\labg}{L^2_{(\aal, \beta, \gamma)}}
\newcommand{\labgn}{L^2_{(\aal + n_1, \beta + n_1, \gamma)}}
\newcommand{\labgnu}{L^2_{(\aal + \nu_1, \beta + \nu_1, \gamma)}}
\newcommand{\nnabg}[1]{\nn{#1}_{L^2_{(\aal, \beta, \gamma)}}}
\newcommand{\genabg}[1]{\left\langle #1 \right\rangle_{\aal, \beta, \gamma}}

%Random Fields
\newcommand{\EE}[1]{\mathbf{E}\left[#1\right]}
\DeclareMathOperator{\Cov}{Cov}


\newcommand{\lom}{{L^2\left(\Om, L^2(\M^d)\right)}}
\newcommand{\lpom}{{L^p\left(\Om, L^2(\M^d)\right)}}
\newcommand{\ltm}{{L^2(\M^d)}}
\newcommand{\ylm}{{Y_\ell^m}}
\newcommand{\xlm}{{X_\ell^m}}
\newcommand{\kiso}{k_{\text{iso}}}
\newcommand{\kis}{K_{\text{IS}}}

%Jacobi Polynomials
\newcommand{\plab}{P_\ell^{(\alpha, \beta)}}
\newcommand{\pkab}{P_{k_1}^{(\alpha, \beta)}}
\newcommand{\hlab}{h_\ell^{(\alpha, \beta)}}
\newcommand{\hkab}{h_{k_1}^{(\alpha, \beta)}}
\newcommand{\wab}{w_{\aal, \beta}}
\newcommand{\rkab}{R^{(\aal, \bb)}_{\mathbf{k}}}

\newcommand{\comm}[1]{\textcolor{magenta}{[#1]}}

\newcommand{\pr}[1]{\mathbf{P}\left(#1\right)}
\newcommand{\expp}[1]{\exp\left(#1\right)}

% Percolation
\newcommand{\pp}{\mathbf{P}_p}
\newcommand{\ppt}{\tilde{\mathbf{P}}_p}
\newcommand{\lr}{\leftrightarrow}
\newcommand{\one}{\mathbf{1}}

% Mixing Times
\newcommand{\tmix}{t_{\text{mix}}}
\newcommand{\nntv}[1]{\nn{#1}_\text{TV}}
\newcommand{\iid}{\stackrel{\text{iid}}{\sim}}
\newcommand{\var}{\text{Var}}

% Advanced Probability
\newcommand{\ctm}{(X_t)_{t \geq 0}}
\newcommand{\fil}{(\cF_t)_{t \geq 0}}
\newcommand{\bm}{\text{BM}}

%SLE
\newcommand{\db}{\overline{\mathbf{D}}}
\let\Im\relax\DeclareMathOperator{\Im}{Im}
\let\Re\relax\DeclareMathOperator{\Re}{Re}
\DeclareMathOperator{\hcap}{hcap}
\DeclareMathOperator{\rad}{rad}
\DeclareMathOperator{\diam}{diam}

%Stochastic Calculus
\DeclareMathOperator{\sgn}{sgn}
\newcommand{\nnn}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}

%SLE
\newcommand{\cci}{C_c^\infty(D)}
\newcommand{\gend}[1]{{\left\langle #1 \right\rangle}_\nabla}
\newcommand{\hz}{H_0^1(D)}
\newcommand{\slek}{\text{SLE}_\kappa}
\newcommand{\slef}{\text{SLE}_4}
\newcommand{\slefr}{\text{SLE}_4(\rho_L ; \rho_R)}
\newcommand{\slekr}{\text{SLE}_\kk(\underline{\rho})}

%Conformal Removability
\DeclareMathOperator{\dqh}{dist_{\text{qh}}}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\Bin}{Bin}
\DeclareMathOperator{\bern}{Bernoulli}


\newcommand{\dqhz}{\dqh(z_0, \cdot)}
\newcommand{\dqz}[1]{\dqh(z_0, #1)}
\newcommand{\tell}{\tilde{\ell}}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\td}{\tilde{D}}
\newcommand{\rn}[1]{\llbracket #1 \rrbracket}
\newcommand{\ci}{\C_\infty}

\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\wh}[1]{\widehat{#1}}


